Investigating social alignment via mirroring in a system of interacting language models

Alignment is a social phenomenon wherein individuals share a common goal or perspective. Mirroring, or mimicking the behaviors and opinions of another individual, is one mechanism by which individuals can become aligned. Large scale investigations of the effect of mirroring on alignment have been limited due to the scalability of traditional experimental designs in sociology. In this paper, we introduce a simple computational framework that enables studying the effect of mirroring behavior on alignment in multi-agent systems. We simulate systems of interacting large language models in this framework and characterize overall system behavior and alignment with quantitative measures of agent dynamics. We find that system behavior is strongly influenced by the range of communication of each agent and that these effects are exacerbated by increased rates of mirroring. We discuss the observed simulated system behavior in the context of known human social dynamics.

==> text/pnas_intro.tex <==
\dropcap{A} key phenomenon underlying the formation of human groups is social alignment \cite{Ransom}. 
This phenomenon, through which individuals adopt the behaviors of the individuals they interact with, has been shown to support the creation of social relationships through the promotion of positive commonality \cite{ACM}. 
In short, like attracts like, and it is through social alignment that individuals behave more alike one another in order to foster cohesive relationships. 

One of the most direct mechanisms to achieve social alignment is social mirroring \cite{Hasson_Frith_2016a}. This occurs primarily subconsciously, as individuals will mimic (or mirror) the facial expressions, posture, mannerisms, and other behaviors of those with whom they interact \cite{bahar}. However, social mirroring is not limited to physical mimicry, as it can also include a more complete degree of copying wherein individuals parrot speech patterns, opinions, and perspectives of those they are mirroring to appear maximally agreeable  \cite{Byrne_2005}. 

While social mirroring has been studied extensively in small group conditions -- primarily with respect to one-on-one interacting pairs \cite{galloti} -- little research has been done exploring its system-level consequences, primarily due to the infeasibility of large-scale experiments. Instead, system-level social science research has been predominantly concerned with the broad consequences of social alignment in group performance once a group has already been established \cite{local_alignment}, rather than the decentralized processes from which those groups can emerge. 

% of the effects of mirroring on pairwise alignment and entire system evolution.
% To that end, we design and deploy a system of interacting LLMs which mimic the means by which humans share, copy, and adopt information. 

Previous theoretical work exploring foundational human social behaviors has been conducted through either purely mathematical means such as the long-tested voter model of population dynamics \cite{redner} or via overly simple computational frameworks \cite{doi:10.1073/pnas.2106292118}. While these approaches can produce excellent insights into the general social dynamics of a population, recent advances in machine learning techniques have enabled explorations of classic economic, psycholinguistic, and social psychology experiments. 
For example, the recent cohort of Large Language Models (LLMs), such as OpenAI's GPT4, are able to replicate the Ultimatum Game, Garden Path Sentences, and Milgram Shock Experiment \citep{aher}. 

Although recent LLMs are able to generate human-like outputs \citep{webb, helm2023statisticalturingtestgenerative} and replicate classic experiments without explicit training (see, e.g., \cite{webb}), human-like behavior is not sufficient to model individuals in a social system.
Indeed, it is necessary to have generative variation across agents that effectively mimics cognitive differences across people.
% it is necessary to have diversity in generative model behavior when using LLMs to study the behaviors of individuals in social communities.
% Although some studies claim that recent LLMs are able to generate human-like outputs without explicit training (see, e.g., \cite{webb}), using one foundational generative model for all LLM agents is insufficient when studying behaviors of social communities through a system of LLMs, as the differentiation of agents is crucial to successfully modeling cognitive differences between people. 
% Hence, we equip LLMs with different external databases and simple associated retrieval mechanisms to promote diverse and individualized responses.
% Retrieval-Augmented Generation (RAG) databases. 
Prior research has shown that retrieval augmented generation (``RAG") improves the performance of LLMs by allowing them to retrieve documents that are relevant to a query from a domain-specific or knowledge-intensive database \citep{rag}. 
For social experiments, a RAG database can be considered the knowledge base or memory of an individual in the social system: the LLM will generate responses based on the combination of its pre-training data and the RAG database, just as people express their thoughts based on a history of previous experiences and the current environmental context.
Previous work studying LLM agents, such as \cite{park2023generative}, have shown that pairing a single LLM with a RAG database-per-individual can effectively promote generation diversity.
% Also mention LLM agent-based simulations where the analysis is focused on individual polarization instead of understand macro/system-level characteristics 

In this paper we present a computational framework to study the macroscopic effects of social alignment through social mirroring. Our framework is parameterized by important characteristics of interactions in a social system, such as the likelihood of an individual being mirrored and the range of individuals with whom someone may interact.
The framework is general to collections of agents that have the capacity to exchange information, though our analysis focuses on systems of interacting LLMs due to their ability to exchange information in natural language at a human-like capacity.

We first introduce our experiment of interacting LLMs to study the effect of mirroring on social alignment in detail. 
We then present and discuss the results before interpreting them from the perspective of comparable social science case studies.

\begin{figure*}[t]
\centering
    \includegraphics[width=\linewidth]{figures/pnas_plot.pdf}
    \caption{Illustration of simulated system dynamics with $ n = 7 $ agents with a communication range of $ k = 3 $. 
    Dashed arrows connect agents in the communication range of the receiving agent. 
    Solid arrows connect the agent that interacted with the receiving agent.
    Arrow color represents the type of interaction -- if it is the color of the receiving agent then communicating agent is mirroring, otherwise they are not mirroring.
    Mirorring occurs with probability $ p $ for each interaction.
    The opinion of an agent and the agents in its range of communication may change at time $ t + 1 $ based off its interaction at time $ t $.
    For example, the blue arrow from the light-blue male to the orange female at $ t $ affects the opinion of the orange female at $ t + 1 $ -- she becomes light blue and the agents in her communication range change.
    See Section \ref{sec:mechanics} for further details.}
\label{fig:system_illustration}
\end{figure*}
